Towards AI-Assisted Synthesis of Verified Dafny Methods

Large language models show great promise in many domains, including programming. A promise is easy to make but hard to keep, and language models often fail to keep their promises, generating erroneous code. A promising avenue to keep models honest is to incorporate formal verification: generating programs' specifications as well as code so that the code can be proved correct with respect to the specifications. Unfortunately, existing large language models show a severe lack of proficiency in verified programming. In this paper, we demonstrate how to improve two pretrained models' proficiency in the Dafny verification-aware language. Using 178 problems from the MBPP dataset, we prompt two contemporary models (GPT-4 and PaLM-2) to synthesize Dafny methods. We use three different types of prompts: a direct Contextless prompt; a Signature prompt that includes a method signature and test cases, and a Chain of Thought (CoT) prompt that decomposes the problem into steps and includes retrieval augmentation generated example problems and solutions. Our results show that GPT-4 performs better than PaLM-2 on these tasks and that both models perform best with the retrieval augmentation generated CoT prompt. GPT-4 was able to generate verified, human-evaluated, Dafny methods for 58% of the problems, however, GPT-4 managed only 19% of the problems with the Contextless prompt, and even fewer (10%) for the Signature prompt. We are thus able to contribute 153 verified Dafny solutions to MBPP problems, 50 that we wrote manually, and 103 synthesized by GPT-4. Our results demonstrate that the benefits of formal program verification are now within reach of code generating large language models...

==> code/exmp_1.tex <==
\begin{lstlisting}[style = mystyle, frame=tb, caption=A simple example program in Dafny, label=lst:example]
method SwapFirstAndLast(a: array<int>)
    requires a.Length > 0
    modifies a
    ensures a[0] == old(a[a.Length - 1])
    ensures a[a.Length - 1] == old(a[0])
    ensures forall k :: 1 <= k < a.Length - 1 ==> a[k] == old(a[k])
{
    var tmp := a[0];
    a[0] := a[a.Length - 1];
    a[a.Length - 1] := tmp;
}
\end{lstlisting}

==> code/exmp_2.tex <==
\begin{tcolorbox}
[
    width=0.67\textwidth, 
    colframe=black, 
    colback=anti-flashwhite!0, 
    boxsep=1mm, 
    arc=1mm,
    title={Direct Prompt},
    skin=bicolor,
    bottom=0mm,
    fontupper=\scriptsize
]
\begin{lstlisting}[style = mystyle, frame=none, label=lst:example, basicstyle=\small]
method FindSmallest(s: array<int>) returns (min: int)
    // preconditions
    requires s.Length > 0 
    // postconditions
    ensures forall i :: 0 <= i < s.Length ==> min <= s[i]   
    ensures exists i :: 0 <= i < s.Length && min == s[i]
{
    min := s[0];
    for i := 1 to s.Length
        //loop-invariants
        invariant 0 <= i <= s.Length  
        invariant forall k :: 0 <= k < i ==> min <= s[k]
        invariant exists k :: 0 <= k < i && min == s[k]
    {
        if s[i] < min { min := s[i]; }        
    }
}
/*Main program, with a simple test case 
(checked statically!).*/

method Main() {
    var a1:= new int[] [1,2,3];
    var out1:= FindSmallest(a1);
    assert out1 == 1;
}
\end{lstlisting}
\end{tcolorbox}

==> code/inv/iv1.tex <==
method RemoveChars(s1: string, s2: string) returns (v: string)
    ensures |v| <= |s1|
    ensures forall i :: 0 <= i < |v| ==> (v[i] in s1) && !(v[i] in s2)
    ensures forall i :: 0 <= i < |s1| ==> (s1[i] in s2) || (s1[i] in v)
{
    var v' : string := [];
    for i := 0 to |s1|
    invariant 0 <= i <= |s1|
    invariant |v'| <= i
    invariant forall k :: 0 <= k < |v'| ==> (v'[k] in s1) && !(v'[k] in s2)
    invariant forall k :: 0 <= k < i ==> (s1[k] in s2) || (s1[k] in v')
    {
        if !(s1[i] in s2)
        {
            v' := v' + [s1[i]];
        }
    }
    return v';
}

==> code/module/577_modul_gpt_rq3.tex <==
Write a method in Dafny to find the factorial of the last digit in a given number. 


function Factorial(n: int): int
    requires n >= 0
    ensures 0 <= Factorial(n)
    {
        if n == 0 then 1
        else n * Factorial(n-1)
    }

    method FactorialOfLastDigit(n: int) returns (fact: int)
    requires n >= 0
    ensures fact == Factorial(n % 10)
    {
        var lastDigit := n % 10;
        fact := Factorial(lastDigit);
    }

==> code/post/578_post_gpt_rq3.tex <==
Write a method in Dafny to interleave 3 sequence of the same length into a single flat sequence.

method Interleave(s1: seq<int>, s2: seq<int>, s3: seq<int>) returns (r: seq<int>)
    requires |s1| == |s2| && |s2| == |s3|
    ensures |r| == 3 * |s1|
    ensures forall i :: 0 <= i < |s1| ==> r[3*i] == s1[i] && r[3*i + 1] == s2[i] && r[3*i + 2] == s3[i]
{
    r := [];
    for i := 0 to |s1|
        invariant 0 <= i <= |s1|
        invariant |r| == 3 * i
        invariant forall k :: 0 <= k < i ==> r[3*k] == s1[k] && r[3*k + 1] == s2[k] && r[3*k + 2] == s3[k]
    {
        r := r + [s1[i], s2[i], s3[i]];
    }
}

==> code/post/586_post_gpt_rq3.tex <==
Write a method in Dafny to split a list at the nth element and add the first part to the end.
WEAK One of the postconditions is missing. Good example.



method SplitAndAppend(l: seq<int>, n: int) returns (r: seq<int>)
    requires n >= 0 && n < |l|
    ensures |r| == |l|
    ensures forall i :: 0 <= i < |l| ==> r[i] == l[(i + n) \% |l|]
{
    var firstPart: seq<int> := l[..n];
    var secondPart: seq<int> := l[n..];
    r := secondPart + firstPart;
}

==> code/post/751_post_gpt_rq3.tex <==
Write a method in Dafny to check if the given array represents min heap or not.


method IsMinHeap(a: array<int>) returns (result: bool)
    requires a != null
    ensures result ==> forall i :: 0 <= i < a.Length / 2 ==> a[i] <= a[2*i + 1] && (2*i + 2 == a.Length || a[i] <= a[2*i + 2])
    ensures !result ==> exists i :: 0 <= i < a.Length / 2 && (a[i] > a[2*i + 1] || (2*i + 2 != a.Length && a[i] > a[2*i + 2]))
{
    result := true;
    for i := 0 to a.Length / 2
        invariant 0 <= i <= a.Length / 2
        invariant result ==> forall k :: 0 <= k < i ==> a[k] <= a[2*k + 1] && (2*k + 2 == a.Length || a[k] <= a[2*k + 2])
    {
        if a[i] > a[2*i + 1] || (2*i + 2 != a.Length && a[i] > a[2*i + 2]) {
            result := false;
            break;
        }
    }
}

==> code/post/post_strong_2.tex <==
// Write a method in Dafny to calculate the sum of the negative numbers of a given list of numbers.

function sumNegativesTo( a:array<int>, n:int ) : int
  requires a != null;
  requires 0 <= n && n <= a.Length;
  decreases n;
  reads a;
{
  if (n == 0) then 0 else if a[n-1] < 0 
              then sumNegativesTo(a, n-1) + a[n-1] else sumNegativesTo(a, n-1)
}

method SumOfNegatives(a: array<int>) returns (result: int)
    ensures result == sumNegativesTo(a, a.Length)

==> code/post/post_weak.tex <==
\begin{lstlisting}[style = mystyle, frame=none]
/*Write a (*@\textcolor{dkgreen}{method}@*) in Dafny to split a list at the nth element 
and add the first part to the end.*/
method SplitAndAppend(l: seq<int>, n: int) returns (r: seq<int>)
    requires n >= 0 && n < |l|
    ensures |r| == |l|
    ensures forall i :: 0 <= i < |l| ==> r[i] == l[(i + n) % |l|]
\end{lstlisting}


